PixelRefer: A Unified Framework for Spatio-Temporal Object Referring with Arbitrary Granularity

Multimodal large language models (MLLMs) have demonstrated strong general-purpose capabilities in open-world visual comprehension. However, most existing MLLMs primarily focus on holistic, scene-level understanding, often overlooking the need for fine-grained, object-centric reasoning. In this paper, we present PixelRefer, a unified region-level MLLM framework that enables advanced fine-grained understanding over user-specified regions across both images and videos. Motivated by the observation that LLM attention predominantly focuses on object-level tokens, we propose a Scale-Adaptive Object Tokenizer (SAOT) to generate compact and semantically rich object representations from free-form regions. Our analysis reveals that global visual tokens contribute mainly in early LLM layers, inspiring the design of PixelRefer-Lite, an efficient variant that employs an Object-Centric Infusion module to pre-fuse global context into object tokens. This yields a lightweight Object-Only Framework that substantially reduces computational cost while maintaining high semantic fidelity. To facilitate fine-grained instruction tuning, we curate PixelRefer-2.2M, a high-quality object-centric instruction dataset. Extensive experiments across a range of benchmarks validate that PixelRefer achieves leading performance with fewer training samples, while PixelRefer-Lite offers competitive accuracy with notable gains in efficiency.

==> sec/2_relatedwork.tex <==

\section{Related Work}
\noindent 
Related Work.

==> sec/3_method.tex <==
\section{Methodology}
\noindent
Methodology.

==> sec/4_experiment.tex <==
\begin{table*}
\centering
\scriptsize
\caption{\textbf{Comparison with diffusion models on ImageNet of 256$\times$256 and 512$\times$512 resolutions}. \textbf{Bold font} and \underline{underline} denote the best and the second-best performance, respectively.
}

\tablestyle{10pt}{1.1}
 \begin{tabular}
{c  c c c c c c  c }
    Model & Params. (M) $\downarrow$   & FLOPs (G) $\downarrow$  & FID $\downarrow$ & sFID $\downarrow$ & IS $\uparrow$ & Precision $\uparrow$ & Recall $\uparrow$ \\
  \midrule[1.2pt]
  \multicolumn{8}{c}{\emph{Static $256 \times 256$}} \\
    ADM & 608 & 1120 & 4.59 & 5.25 & 186.87 & 0.82 & 0.52 \\
    % LDM-8 & 395 & 57 & 7.76 & - & 209.52 & 0.84 & 0.35 \\
    LDM-4 & 400 & 104 & 3.95 & - & 178.22 & 0.81 & 0.55 \\
    U-ViT-L/2 & \textbf{287} & \underline{77} & 3.52 & - & - & - & -  \\
    U-ViT-H/2 & 501 & 113 & 2.29 & - & 247.67 & \textbf{0.87} & 0.48  \\
    DiffuSSM-XL & 673 & 280 & 2.28 & \textbf{4.49} & 269.13 &\underline{0.86} & 0.57 \\
    DiM-L & \underline{380} & 94 & 2.64 & - & - & - & - \\
    DiM-H & 860 & 210 & 2.21 & - & - & - & - \\
    DiffiT  &  561 & 114	& \underline{1.73} & - &276.49 & 0.80 & \underline{0.62} \\ 
    % SiT-XL  &  675 & 118	&2.06 &\textbf{4.49} &277.50 &0.83 &0.59 \\
    DiMR-XL & 505 & 160 & \textbf{1.70} & -& \textbf{289.00} & 0.79 & \textbf{0.63}\\
    \hshline
    DiT-L & 468 & 81 & 5.02 &- & 167.20 & 0.75 & 0.57 \\
    DiT-XL & 675 & 118 & 2.27 & 4.60 & 277.00 & 0.83 & 0.57 \\ 
\hshline
        


\multicolumn{8}{c}{\emph{Dynamic $256 \times 256$}} \\
   \rowcolor{gray!15} DyDiT-XL$_{\lambda=0.7}$ &  678 & 84.33 (\textcolor{blue}{$\downarrow$1.40$\times$})  & 2.12 & 4.61 & \underline{284.31} & 0.81 & 0.60  \\
   \rowcolor{gray!15} DyDiT-XL$_{\lambda=0.5}$ &  678 & \textbf{57.88  (\textcolor{blue}{$\downarrow$2.04$\times$})}  & 2.07 & \underline{4.56} & 248.03 & 0.80 & 0.61  \\ 

  \midrule[1.2pt]
  \multicolumn{8}{c}{\emph{Static $512 \times 512$}}\\

ADM-G	& 731	& 2813	& 3.85	& 5.86 & 221.72	& \underline{0.84}	& 0.53 \\
DiffuSSM-XL & 673	& 1066	& 3.41	& -	& \textbf{255.00}	& \textbf{0.85} & 0.49 \\
DiM-Huge	&	860	& 708	&3.78	&-	&-	&-	& - \\ \hshline

DiT-XL & \textbf{675}	& \underline{514}	& 3.04	& \textbf{5.02}	& \underline{240.80}	& \underline{0.84}	& \underline{0.54} \\ \hshline

\multicolumn{8}{c}{\emph{Dynamic $512 \times 512$}}\\
 \rowcolor{gray!15} DyDiT-XL$_{\lambda=0.7}$ &  \underline{678} & \textbf{375.05 (\textcolor{blue}{$\downarrow$1.37$\times$})}	& \textbf{2.88}	& \underline{5.14}	& 228.93	& 0.83	& \textbf{0.56}  \\

   
\end{tabular}
\label{tab:sota}
\vspace{-2mm}
\end{table*}









\begin{figure*}[htbp]
    \centering
    % 第一列子图
    \includegraphics[width=0.337\textwidth]{figures/flops/DiT-S_flops_fid.pdf}
    \hfill % 子图间的弹性间距
    % 第二列子图
    \includegraphics[width=0.321\textwidth]{figures/flops/DiT-B_flops_fid.pdf}
    \hfill % 子图间的弹性间距
    % 第三列子图
    \includegraphics[width=0.325\textwidth]{figures/flops/DiT-XL_flops_fid.pdf}
    % \vskip -0.05in
    \caption{\textbf{FLOPs-FID trade-off on ImageNet.}}
    \label{fig:flops_fid_figure}
    % \vskip -0.05in
\end{figure*}

\section{Experiments}
\noindent
Experiments showed in Table~\ref{tab:sota} and Figure~\ref{fig:flops_fid_figure}.

==> sec/5_conclusion.tex <==
\section{Discussion and Conclusion}
\noindent


Conclusion here.








==> sec/6_ack.tex <==
\section*{Acknowledgement}
The LaTeX template is built upon Meta’s original template.
